On the energetic analysis of autonomous quantum systems

In this thesis, we focus on the energetic analysis within autonomous quantum systems. To this aim, we propose a novel and general formalism for a dynamic description of the energy exchanges between interacting subsystems. From the Schmidt decomposition approach, we identify effective Hamiltonians as the representative operators for characterizing the local internal energies, whose expectation values satisfy the usual thermodynamic notion of energy additivity. In contrast to the currently used methodologies, such procedure treats the subsystems with equal footing and do not rely on any sort of approximations and additional hypotheses, e.g., semi-classical description, weak-coupling regime, strict energy conservation and Markovian dynamics. In short, our proposal contributes to the development of QT by providing a new formalism that does not suffer from the usual restrictive shortcomings and establishes a new and exact route for defining other general thermodynamic quantities to the quantum regime.

==> Outros/USPSC-Apendices.tex <==
%% USPSC-Apendice.tex
% ---
% Inicia os apêndices
% ---

\begin{apendicesenv}
% Imprime uma página indicando o início dos apêndices
\partapendices
\chapter{Schmidt decomposition}



% ----------------------------------------------------------
\chapter{Exemplo de tabela com grade}
\index{tabelas}A \autoref{tab-grade} exemplifica a inclusão de traços estruturadores de conteúdo para melhor compreensão do conteúdo da tabela, em conformidade com as normas de apresentação tabular do IBGE.
% utilize \usepackage{array} no PREAMBULO (ver em USPSC-modelo.tex) obter uma tabela centralizada verticalmente e horizontalmente
\begin{table}[htb]
\ABNTEXfontereduzida
\caption[Exemplo de tabelas com grade]{Exemplo de tabelas com grade}
\label{tab-grade}
\begin{tabular}{ >{\centering\arraybackslash}m{8cm} | >{\centering\arraybackslash}m{6cm} }
\hline
 \centering \textbf{Coluna A} & \textbf{Coluna B}\\
\hline
  A1 & B1\\
\hline
  A2 & B2\\
\hline
  A3 & B3\\
\hline
  A4 & B4\\
\hline
\end{tabular}
\begin{flushleft}
		Fonte: Elaborada pelos autores.\
\end{flushleft}
\end{table}


\end{apendicesenv}
% ---

==> USPSC-fichacatalografica.tex <==
% ---
% Inserir a ficha bibliografica
% ---
% Isto é um exemplo de Ficha Catalográfica, ou ``Dados internacionais de
% catalogação-na-publicação''. Você pode utilizar este modelo como referência. 
% Porém, provavelmente a biblioteca da sua universidade lhe fornecerá um PDF
% com a ficha catalográfica definitiva após a defesa do trabalho. Quando estiver
% com o documento, salve-o como PDF no diretório do seu projeto e substitua todo
% o conteúdo de implementação deste arquivo pelo comando abaixo:
%
\begin{fichacatalografica}
	\hspace{-1.4cm}
	\imprimirnotaautorizacao \\ \\
	%\sffamily
	\vspace*{\fill}					% Posição vertical
	\begin{center}					% Minipage Centralizado
		\imprimirnotabib \\
\begin{table}[htb]
	\scriptsize
	\centering	
	\begin{tabular}{|p{0.9cm} p{8.7cm}|}
		\hline
	      & \\
		  &	  \imprimirautorficha     \\
		
		 \imprimircutter & 
							\hspace{0.4cm}\imprimirtitulo~  / ~\imprimirautor~ ;  ~\imprimirorientadorcorpoficha. -- 	\imprimirlocal, \imprimirdata.   \\
		
		  &  % Para incluir nota referente à versão corrigida no corpo da ficha,
			  % incluir % no início da linha acima e tirar a % do início da linha abaixo
			  %	\hspace{0.4cm} \imprimirtitulo~  / ~\imprimirautor~ ; ~\imprimirorientadorcorpoficha~- ~\imprimirnotafolharosto. -- \imprimirlocal, \imprimirdata.  \\
		
			\hspace{0.4cm}\pageref{LastPage} p. : il. (algumas color.) ; 30 cm.\\ 
		  & \\
		  & 
		    \hspace{0.4cm}\imprimirnotaficha ~--~ 
						  \imprimirunidademin, 
						  \imprimiruniversidademin, 
		                  \imprimirdata. \\ 
		  & \\                 
		   % Para incluir nota referente à versão corrigida em notas,
		    % incluir uma % no início da linha acima e	
		    % tirar a % do início da linha abaixo
		    % & \hspace{0.4cm}\imprimirnotafolharosto \\ 
		  & \\ 
		  & \hspace{0.4cm}1. LaTeX. 2. abnTeX. 3. Classe USPSC. 4. Editoração de texto. 5. Normalização da documentação. 6. Tese. 7. Dissertação. 8. Documentos (elaboração). 9. Documentos eletrônicos. I. \imprimirorientadorficha. 
		   II. Título. \\
	
		     %Se houver co-orientador, inclua % antes da linha (antes de II. Título.) 
		     %          e tire a % antes do comando abaixo 
		     %III. Título. \\   
		  \hline
	\end{tabular}
\end{table}
	\end{center}
\end{fichacatalografica}
% ---



==> USPSC-pre-textual-IFSC.tex <==
%% USPSC-pre-textual-IFSC.tex
%% Camandos para definição do tipo de documento (tese ou dissertação), área de concentração, opção, preâmbulo, titulação 
%% referentes ao Programa de Pós-Graduação o IFSC
\instituicao{Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo}
\unidade{INSTITUTO DE F\'ISICA DE S\~AO CARLOS}
\unidademin{Instituto de F\'isica de S\~ao Carlos}
\universidademin{Universidade de S\~ao Paulo}

%\notafolharosto{Vers\~ao original}
%Para versão original em inglês, comente do comando/declaração 
%     acima(inclua % antes do comando acima) e tire a % do 
%     comando/declaração abaixo no idioma do texto
%\notafolharosto{Original version}
 
%Para versão corrigida, comente do comando/declaração da 
%     versão original acima (inclua % antes do comando acima) 
%     e tire a % do comando/declaração de um dos comandos 
%     abaixo em conformidade com o idioma do texto
%\notafolharosto{Vers\~ao corrigida \\(Vers\~ao original dispon\'ivel na Unidade que aloja o Programa)}
\notafolharosto{Corrected version \\(Original version available on the Program Unit)}

% Para utilizar Sistema Numérico diferente da ABNT
% Numeração entre colchetes:
%\citebrackets[] 
% Numeração entre parenteses:

% ---
% dados complementares para CAPA e FOLHA DE ROSTO
% ---
\universidade{UNIVERSIDADE DE S\~AO PAULO}
\titulo{On the energetic analysis of autonomous quantum
systems}
% Se o idioma do texto for o inglês, inclua % antes da linha acima e retire a % da linha abaixo
%\titulo{Model for thesis and dissertations in \LaTeX\ using the USPSC Package to the IFSC}

\titleabstract{On the energetic analysis of autonomous quantum systems}
\tituloresumo{Sobre a análise energética de sistemas quânticos autônomos}
\autor{André Hernandes Alves Malavazi}
\autorficha{Malavazi, André Hernandes Alves}
\autorabr{MALAVAZI, A. H. A.}

\cutter{S856m}
% Para gerar a ficha catalográfica sem o Código Cutter, basta 
% incluir uma % na linha acima e tirar a % da linha abaixo
%\cutter{ }

\local{S\~ao Carlos}
\data{2022}
% Quando for Orientador, basta incluir uma % antes do comando abaixo
\renewcommand{\orientadorname}{Orientador:}
% Quando for Coorientadora, basta tirar a % utilizar o comando abaixo
%\newcommand{\coorientadorname}{Coorientador:}
\orientador{Prof. Dr. Frederico Borges de Brito}
\orientadorcorpoficha{orientadora Frederico Borges de Brito}
\orientadorficha{de Brito, Frederico Borges, orient}
%Se houver co-orientador, inclua % antes das duas linhas (antes dos comandos \orientadorcorpoficha e \orientadorficha) 
%          e tire a % antes dos 3 comandos abaixo
%\coorientador{Prof. Dr. Jo\~ao Alves Serqueira}
%\orientadorcorpoficha{orientadora Elisa Gon\c{c}alves Rodrigues ;  co-orientador Jo\~ao Alves Serqueira}
%\orientadorficha{Rodrigues, Elisa Gon\c{c}alves, orient. II. Serqueira, Jo\~ao Alves, co-orient}

\notaautorizacao{AUTORIZO A REPRODU\c{C}\~AO E DIVULGA\c{C}\~AO TOTAL OU PARCIAL DESTE TRABALHO, POR QUALQUER MEIO CONVENCIONAL OU ELETR\^ONICO PARA FINS DE ESTUDO E PESQUISA, DESDE QUE CITADA A FONTE.}
% Se o idioma for o inglês, inclua a % antes do campo \notaautorizacao acima e retire a % da linha abaixo
%\notaautorizacao{I AUTORIZE THE REPRODUCTION AND DISSEMINATION OF TOTAL OR PARTIAL COPIES OF THIS DOCUMENT, BY CONVENCIONAL OR ELECTRONIC MEDIA FOR STUDY OR RESEARCH PURPOSE, SINCE IT IS REFERENCED.}
\notabib{Ficha catalogr\'afica revisada pelo Servi\c{c}o de Biblioteca e Informa\c{c}\~ao Prof. Bernhard Gross, com os dados fornecidos pelo(a) autor(a)}

\newcommand{\programa}[1]{

% DFAp ==========================================================================
\ifthenelse{\equal{#1}{DFAp}}{
    \tipotrabalho{Tese (Doutorado em Ci\^encias)}
    \tipotrabalhoabs{Thesis (Doctor in Science)}
    \area{F\'isica Aplicada}
	%\opcao{Nome da Opção}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% DFAe ==========================================================================
\ifthenelse{\equal{#1}{DFAe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{Applied Physics}
	%\opcao{Nome da Opção}
   	% O preambulo deve conter o tipo do trabalho, o objetivo, 
   	% o nome da instituição, a área de concentração e opção quando houver
   	\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
   	\notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
    }{    
% MFAp ===========================================================================
\ifthenelse{\equal{#1}{MFAp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Aplicada}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% MFAe ===========================================================================
\ifthenelse{\equal{#1}{MFAe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{Applied Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of  Master in Science.}
	\notaficha{Dissertation (Master - Graduate Program in Applied Physics)}	
    }{        
% DFAFCp ==========================================================================
\ifthenelse{\equal{#1}{DFAFCp}}{
    \tipotrabalho{Tese (Doutorado em Ci\^encias)}
    \tipotrabalhoabs{Thesis (Doctor in Science)}
    \area{F\'isica Aplicada}
    \opcao{F\'isica Computacional}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% DFAFCe ==========================================================================
\ifthenelse{\equal{#1}{DFAFCe}}{
    \renewcommand{\areaname}{Concentration area:}
    \renewcommand{\opcaoname}{Option:}
    \renewcommand{\orientadorname}{Advisor:}
    \tipotrabalho{Tese (Doutorado em Ci\^encias)}
    \tipotrabalhoabs{Thesis (Doctor in Science)}
   	\area{Applied Physics}
    \opcao{Computational Physics}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
    % o nome da instituição, a área de concentração e opção quando houver
    \preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
    \notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
    }{
% MFAFCp ===========================================================================
\ifthenelse{\equal{#1}{MFAFCp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Aplicada}
	\opcao{F\'isica Computacional}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% MFAFCe ===========================================================================
\ifthenelse{\equal{#1}{MFAFCe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{Applied Physics}
	\opcao{Computational Physics}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of  Master in Science.}
	\notaficha{Dissertation (Master - Graduate Program in Applied Physics)}
    }{
% DFAFBp ===========================================================================
\ifthenelse{\equal{#1}{DFAFBp}}{
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{F\'isica Aplicada}
	\opcao{F\'isica Biomolecular}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{				
% DFAFBe ===========================================================================
\ifthenelse{\equal{#1}{DFAFBe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{Applied Physics}
	\opcao{Biomolecular Physics}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
	\notaficha{Thesis (Doctorate - Graduate Program in Applied Physics)}
    }{				
% MFAFBp ===========================================================================
\ifthenelse{\equal{#1}{MFAFBp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Aplicada}
	\opcao{F\'isica Biomolecular}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Aplicada)}
    }{
% MFAFBe ===========================================================================
\ifthenelse{\equal{#1}{MFAFBe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{Applied Physics}
	\opcao{Biomolecular Physics}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
	\notaficha{Dissertation (Master - Graduate Program in Applied Physics}
    }{				
% DFBp ==========================================================================
\ifthenelse{\equal{#1}{DFBp}}{
    \tipotrabalho{Tese (Doutorado em Ci\^encias)}
    \tipotrabalhoabs{Thesis (Doctor in Science)}
    \area{F\'isica B\'asica}
	%\opcao{Nome da Opção}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
    }{
% DFBe ==========================================================================
\ifthenelse{\equal{#1}{DFBe}}{
    \renewcommand{\areaname}{Concentration area:}
    \renewcommand{\opcaoname}{Option:}
    \renewcommand{\orientadorname}{Advisor:}
    \tipotrabalho{Tese (Doutorado em Ci\^encias)}
    \tipotrabalhoabs{Thesis (Doctor in Science)}
    \area{Basic Physics}
    %\opcao{Nome da Opção}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
    % o nome da instituição, a área de concentração e opção quando houver				
    \preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
    \notaficha{Thesis (Doctorate - Graduate Program in Basic Physics)}
    }{
% MFBp ===========================================================================
\ifthenelse{\equal{#1}{MFBp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica B\'asica}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica B\'asica)}
    }{                
% MFBe ===========================================================================
\ifthenelse{\equal{#1}{MFBe}}{
    \renewcommand{\areaname}{Concentration area:}
    \renewcommand{\opcaoname}{Option:}
    \renewcommand{\orientadorname}{Advisor:}
    \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
    \tipotrabalhoabs{Dissertation (Master in Science)}
    \area{Basic Physics}
    %\opcao{Nome da Opção}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
    % o nome da instituição, a área de concentração e opção quando houver				
    \preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
    \notaficha{Dissertation (Master - Graduate Program in Basic Physics)}
    }{   
% DFBMp ===========================================================================
\ifthenelse{\equal{#1}{DFBMp}}{
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{F\'isica Biomolecular}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Biomolecular)}
    }{   
% DFBMe ===========================================================================
\ifthenelse{\equal{#1}{DFBMe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{Biomolecular Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
	\notaficha{Thesis (Doctorate - Graduate Program in Biomolecular Physics)}
    }{    
% MFBMp ===========================================================================
\ifthenelse{\equal{#1}{MFBMp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Biomolecular}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Biomolecular)}
    }{ 
% MFBMe ===========================================================================
\ifthenelse{\equal{#1}{MFBMe}}{
    \renewcommand{\areaname}{Concentration area:}
    \renewcommand{\opcaoname}{Option:}
    \renewcommand{\orientadorname}{Advisor:}
    \tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
    \tipotrabalhoabs{Dissertation (Master in Science)}
    \area{Biomolecular Physics}
    %\opcao{Nome da Opção}
    % O preambulo deve conter o tipo do trabalho, o objetivo, 
    % o nome da instituição, a área de concentração e opção quando houver				
    \preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
    \notaficha{Dissertation (Master - Graduate Program in Biomolecular Physics)}	
    }{ 
% DFCp ==========================================================================
\ifthenelse{\equal{#1}{DFCp}}{
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{F\'isica Computacional}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Computacional)}
    }{ 
% DFCe ==========================================================================
\ifthenelse{\equal{#1}{DFCe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{Computational Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
	\notaficha{Thesis (Doctorate - Graduate Program in Computational Physics)}
    }{ 
% MFCp ===========================================================================
\ifthenelse{\equal{#1}{MFCp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Computacional}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Computacional)}
    }{ 
% MFCe ===========================================================================
\ifthenelse{\equal{#1}{MFCe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{Computational Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
	\notaficha{Dissertation (Master - Graduate Program in Computational Physics)}	
    }{  
% DFTEp ==========================================================================
\ifthenelse{\equal{#1}{DFTEp}}{
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{F\'isica Te\'orica e Experimental}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Tese apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Doutor em Ci\^encias.}
	\notaficha{Tese (Doutorado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Te\'orica e Experimental)}
    }{
% DFTEe ==========================================================================
\ifthenelse{\equal{#1}{DFTEe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Tese (Doutorado em Ci\^encias)}
	\tipotrabalhoabs{Thesis (Doctor in Science)}
	\area{Theoretical and Experimental Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Thesis presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Doctor in Science.}
	\notaficha{Thesis (Doctorate - Graduate Program in Theoretical and Experimental Physics)}
    }{
% MFTEp ===========================================================================
\ifthenelse{\equal{#1}{MFTEp}}{
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{F\'isica Te\'orica e Experimental}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Disserta\c{c}\~ao apresentada ao Programa de P\'os-Gradua\c{c}\~ao em F\'isica do Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, para obten\c{c}\~ao do t\'itulo de Mestre em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao (Mestrado - Programa de P\'os-Gradua\c{c}\~ao em F\'isica Te\'orica e Experimental)}
    }{  
% MFTEe ===========================================================================
\ifthenelse{\equal{#1}{MFTEe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Disserta\c{c}\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master in Science)}
	\area{Theoretical and Experimental Physics}
	%\opcao{Nome da Opção}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver				
	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
	\notaficha{Dissertation (Master - Graduate Program in Theoretical and Experimental Physics)}		
    }{  
% Outros
	\tipotrabalho{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado)}
	\tipotrabalhoabs{Dissertation/Thesis (Master/Doctor)}
	\area{Nome da \'Area}
	\opcao{Nome da Op\c{c}\~ao}
	% O preambulo deve conter o tipo do trabalho, o objetivo, 
	% o nome da instituição, a área de concentração e opção quando houver
	\preambulo{Disserta\c{c}\~ao/Tese apresentada ao Programa de P\{\o}s-Gradua\c{c}\~ao em F\{\i}sica do Instituto de F\{\i}sica de S\~ao Carlos da Universidade de S\~ao Paulo, para obtenç\c{c}\~ao do t\{\i}tulo de Mestre/Doutor em Ci\^encias.}
	\notaficha{Disserta\c{c}\~ao/Tese (Mestrado/Doutorado - Programa de P\'os-Gradua\c{c}\~ao em Nome da \'Area)}
}}}}}}}}}}}}}}}}}}}}}}}}}}}}}
				
				








==> USPSC-unidades.tex <==
%% USPSC-unidades.tex
% Camando para definição do programa de Pós-Graduação, Especialidade do Título e Instituição
\newcommand{\siglaunidade}[1]{


% EESC-TCC ==========================================================================
    \ifthenelse{\equal{#1}{EESC-TCC}}{
     			\include{USPSC-TCC-pre-textual-EESC}
% ---
    }{
% EESC ==========================================================================
	\ifthenelse{\equal{#1}{EESC}}{
	\include{USPSC-pre-textual-EESC}
	% ---
}{    
% IAU ===========================================================================
        \ifthenelse{\equal{#1}{IAU}}{
        \include{USPSC-pre-textual-IAU}    
        }{
% ICMC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC}}{
        \include{USPSC-pre-textual-ICMC}    
        }{
% ICMC-TCC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC-TCC}}{
        	\include{USPSC-TCC-pre-textual-ICMC}    
        }{
% IFSC ===========================================================================
        \ifthenelse{\equal{#1}{IFSC}}{
        \include{USPSC-pre-textual-IFSC}    
        }{
% IQSC ===========================================================================
        \ifthenelse{\equal{#1}{IQSC}}{
        \include{USPSC-pre-textual-IQSC}    
        }{
% IQSC-TCC ===========================================================================
	\ifthenelse{\equal{#1}{IQSC-TCC}}{
	\include{USPSC-TCC-pre-textual-IQSC}    
       }{
% USPSC ===========================================================================
\ifthenelse{\equal{#1}{USPSC}}{
	\include{USPSC-pre-textual-Tutorial}    
}{
% OUTROS-TCC ===========================================================================
\ifthenelse{\equal{#1}{OUTROS-TCC}}{
	\include{USPSC-TCC-pre-textual-OUTROS}    
}{
% Outros ========================================================================
                       % ------------------------------------------------------------------------
        \include{USPSC-pre-textual-OUTRO} 
								  }
                }
							}
						}
				}
			}}}}}}
         	


==> folhadeaprovacao.tex <==
% Alternativa para a Folha de Aprovação 
% Se esta for a sua opção, exclua inclusão feita acima do arquivo folhadeaprovacao.pdf
%
\begin{folhadeaprovacao}
  \begin{center}
       {\ABNTEXchapterfont\bfseries\large\imprimirautor}
	 \vspace*{2cm}
   
    \begin{center}
      \ABNTEXchapterfont\bfseries\Large\imprimirtitulo
    \end{center}
		\vspace*{2cm}
		\hspace{.45\textwidth}
    \begin{minipage}{.5\textwidth}
        \imprimirpreambulo
    \end{minipage}
		\vspace*{2cm}
    %\vspace*{\fill}
	\end{center}

  \begin{center}
	  {\ABNTEXchapterfont\bfseries\large\ {Data de defesa: 02 de outubro de 2015} \\}
		\vspace*{\fill}
	  {\ABNTEXchapterfont\bfseries\large\ {Comiss\~ao Julgadora:} \\}
		%Trabalho aprovado. \imprimirlocal, 2 de outubro de 2015:
		
		%\assinatura{\textbf{\imprimirorientador} \\ Orientador} 
		\assinatura{\textbf{\imprimirorientador} \\}
    % Se for ORIENTADOR, inclua % no início do comando abaixo e tire a % do próximo comando 
		\renewcommand{\orientadorname}{Orientadora}
		%\renewcommand{\orientadorname}{Orientador}

		\imprimirorientadorRotulo
		\par
		\assinatura{\textbf{Professor} \\ Convidado1}
	
		\assinatura{\textbf{Professor} \\ Convidado2}
		%\assinatura{\textbf{Professor} \\ Convidado3}
		%\assinatura{\textbf{Professor} \\ Convidado4}
		%\begin{center}
		\vspace*{\fill}
   	{\ABNTEXchapterfont\bfseries\large\imprimirlocal}
    \par
    {\ABNTEXchapterfont\bfseries\large\imprimirdata}
\end{center}
\end{folhadeaprovacao}
% ---
